HashCore: Proof-of-Work Functions for General Purpose Processors

Over the past five years, the rewards associated with mining Proof-of-Work blockchains have increased substantially. As a result, miners are heavily incentivized to design and utilize Application Specific Integrated Circuits (ASICs) that can compute hashes far more efficiently than existing general purpose hardware. Currently, it is difficult for most users to purchase and operate ASICs due to pricing and availability constraints, resulting in a relatively small number of miners with respect to total user base for most popular cryptocurrencies. In this work, we aim to invert the problem of ASIC development by constructing a Proof-of-Work function for which an existing general purpose processor (GPP, such as an x86 IC) is already an optimized ASIC. In doing so, we will ensure that any would-be miner either already owns an ASIC for the Proof-of-Work system they wish to participate in or can attain one at a competitive price with relative ease. In order to achieve this, we present HashCore, a Proof-of-Work function composed of "widgets" generated pseudo-randomly at runtime that each execute a sequence of general purpose processor instructions designed to stress the computational resources of such a GPP. The widgets will be modeled after workloads that GPPs have been optimized for, for example, the SPEC CPU 2017 benchmark suite for x86 ICs, in a technique we refer to as inverted benchmarking. We provide a proof that HashCore is collision-resistant regardless of how the widgets are implemented. We observe that GPP designers/developers essentially create an ASIC for benchmarks such as SPEC CPU 2017. By modeling HashCore after such benchmarks, we create a Proof-of-Work function that can be run most efficiently on a GPP, resulting in a more accessible, competitive, and balanced mining market.

==> old_coll_section.tex <==
This section outlines the tests done to measure the security requirements of the widgets. 
Specifically, we require that no two widgets may produce the same output. 
Testing this requirement completely would require generating a widget for every possible input seed, however, testing the complete $2^{256}$ input space is unfeasible. 
To test this requirement initially, we compared the outputs of the thousand different widgets and found that none of the outputs were identical. 
Indeed, if just the output file size was used as the output and the contents ignored, there were still very few collisions between the widgets. 
This supports the idea that the widget generator does not reduce entropy, as the input space is a single 256-bit value and the output space is a 20 to 38 kilobyte value.

We further tested the non-collision by isolating the first register outputs. Mathematically, the probability of two widgets producing the same output is the multiplicative summation of the probability that each register state matches. We analyzed the numerical spread of the first register snapshot for each of the thousand widgets to see if there were any collision and to analyze the value spread. Figure \ref{fig:dist} shows a histogram of this analysis. Each bucket has a range of two million values for the register contents. The most-filled bucket centered around 1.02 Billion has 14 widgets that produced values in that range, and these 14 values differed by roughly one hundred thousand on average. We note that the value spread looks roughly uniform, suggesting that the widgets are producing sufficiently random outputs. Overall, this histogram shows that collisions on even the first register snapshot are highly unlikely, and the probability becomes vanishingly small as more snapshots are considered.

A sampling-theory based argument can also be used to better understand the non-collision property of widgets. The widget generator samples a Gaussian distribution to select instructions while constructing a widget. Thus, the instructions are chosen based on a Gaussian seed, which is non-colliding, rendering the widgets themselves to be transitively non-colliding in nature. Lastly, since the programs are non-colliding, the register outputs are consequently non-colliding as the probability that two independent programs produce the exact same register states is exponentially small. Combined, this results in provably non-colliding, entropy-preserving widgets with high probability.


\begin{figure}[t]
  \centering
  \label{fig:dist}
  \includegraphics[height=0.2\textheight,width=1\linewidth]{Register_Vals.png} 
  \caption{Distribution of Bit Values}
  \vspace{-4mm}
\end{figure}
